On LLR Mismatch in Belief Propagation Decoding of Overcomplete QLDPC Codes

Belief propagation (BP) decoding of quantum low density parity check (QLDPC) codes is often implemented using overcomplete stabilizer (OS) representations, where redundant parity checks are introduced to improve finite length performance. Decoder behavior for such representations is governed primarily by finite iteration dynamics rather than asymptotic code properties. These dynamics are known to critically depend on the initialization of the decoder. In this paper, we investigate the impact of mismatched log likelihood ratios (LLRs) used for BP initialization on the performance of QLDPC codes with OS representations. Our results demonstrate that initial LLR mismatch has a strong influence on the frame error rate (FER), particularly in the low noise regime. We also show that the optimal performance is not sharply localized: the FER remains largely insensitive over an extended region of mismatched LLRs. This behavior motivates an interpretation of LLR mismatch as a regularization control parameter rather than a quantity that must be precisely matched to the quantum channel.

==> figures/tikz_export/Wide_range_Prior_sweep_BP4/fig105.tex <==
% Clean fig105 af the one from matlab was not having good resolution. 
% Had to create the dat files in matlab and brought them here. 
% But in R2017b the export was not working well. 
% patch solution here!
\begin{tikzpicture}[trim axis left, trim axis right]
%%%%%%%%%%%%%%%%%%%%%%
\begin{axis}[
  width=\columnwidth,
  height=0.62\columnwidth,
  xmode=log,
  ymode=log,
  tick label style={font=\scriptsize},
xlabel={epsilon},
ylabel={FER},
xlabel style={
   % font=\bfseries\small
   font=\scriptsize
},
ylabel style={
    font=\scriptsize
},
xlabel style={
  at={(axis description cs:0.5,0.08)},  %-> move up adjust when needed
  anchor=north
},
ylabel style={
  at={(axis description cs:0.08,0.75)},  %
  anchor=south,
  rotate=270
},
  xmin=1e-2, xmax=1e-1,
  grid=major,
  legend pos=south east,
  legend columns=2,
  legend cell align=left,
  legend style={
    font=\tiny,
    draw=none,
    fill=none,
    xshift=10pt
  }
]
% the reading from just one dat file was not working....
%%%%%%%%%%%%%%%%%
  \addplot[thick, solid, red, mark=+, mark size=1pt]
    table {figures/tikz_export/fig105_curves/curve_01.dat};
  \addlegendentry{$\epsilon_{0}$=0.75}
%%%%%%%%%%%%%%%%%
  \addplot[thin, dotted, black, mark=*, mark size=1pt]
    table {figures/tikz_export/fig105_curves/curve_02.dat};
  \addlegendentry{$\epsilon_{0}$=0.12}
%%%%%%%%%%%%%%%%%
  \addplot[thick, solid, blue, mark=+, mark size=1pt]
    table {figures/tikz_export/fig105_curves/curve_03.dat};
  \addlegendentry{$\epsilon_{0}$=0.10}
%%%%%%%%%%%%%%%%%
  \addplot[thin, dotted, blue, mark=square*, mark size=1pt]
    table {figures/tikz_export/fig105_curves/curve_04.dat};
  \addlegendentry{$\epsilon_{0}$=0.091}
%%%%%%%%%%%%%%%%%
  \addplot[thick, dotted, black, mark=triangle*, mark size=1pt]
    table {figures/tikz_export/fig105_curves/curve_05.dat};
  \addlegendentry{$\epsilon_{0}$=0.07}
%%%%%%%%%%%%%%%%%
  \addplot[thin, dashed, black, mark=pentagon*, mark size=1pt]
    table {figures/tikz_export/fig105_curves/curve_06.dat};
  \addlegendentry{$\epsilon_{0}$=0.03}
%%%%%%%%%%%%%%%%%
\end{axis}
\end{tikzpicture}


==> figures/tikz_export/Wide_range_Prior_sweep_BP4/fig2_ep0_opt/fig2.tex <==
% figures/tikz_export/fig2_ep0_opt/fig2.tex is the valid one, final version!
\begin{tikzpicture}
\begin{axis}[
  width=0.95\columnwidth,
  height=0.55\columnwidth,
  grid=both,
  grid style={line width=.1pt, draw=black!15},
  major grid style={line width=.2pt, draw=black!25},
  xlabel={$L_0$ (\,\epsilon_0\ shown below\,)},
  ylabel={$\Delta J(L_0)=J(L_0)-J(L_{0,\mathrm{ref}})$},
  xmin=2.95, xmax=3.60,

  % make it look like MATLAB (no 10^{-2} scaling) 
  scaled y ticks=false,
  yticklabel style={/pgf/number format/fixed, /pgf/number format/precision=3},

  % FORCE limits as this was overdrafting.
  ymin=-0.06, ymax=0.09,

  tick label style={font=\footnotesize},
  label style={font=\footnotesize},
  title style={font=\footnotesize},
  legend style={draw=none, fill=none, font=\footnotesize, cells={anchor=west}},
  legend pos=north east,
  title={Zoomed objective difference around reference},
  xtick={3.0,3.2,3.4,3.6},
  xticklabels={{3.00\\(0.130)},{3.20\\(0.109)},{3.40\\(0.091)},{3.60\\(0.076)}},
  unbounded coords=jump,
]
%%%%%%%%
\pgfplotstableread{figures/tikz_export/fig2_ep0_opt/fig2_data_depured.dat}\Traw
\pgfplotstablesort[sort key=L0]\T{\Traw}
%%%%%%%%% 95% CI band 
\addplot[name path=upper, draw=none] table[x=L0,y=deltaJ_hi] {\T};
\addplot[name path=lower, draw=none] table[x=L0,y=deltaJ_lo] {\T};
\addplot[fill=black!12, draw=none] fill between[of=upper and lower];
\addlegendentry{$95\%$ CI}
% mean curve 
\addplot[black, thick] table[x=L0,y=deltaJ] {\T};
\addlegendentry{mean $\Delta J$}
% markers by cls 
\addplot[only marks, mark=+, mark size=2.3pt, black]
  table[x=L0,y=deltaJ, restrict expr to domain={\thisrow{cls}}{-1:-1}] {\T};
\addlegendentry{$\Delta J<0$ (better)}
\addplot[only marks, mark=x, mark size=2.2pt, black]
  table[x=L0,y=deltaJ, restrict expr to domain={\thisrow{cls}}{1:1}] {\T};
\addlegendentry{$\Delta J>0$ (worse)}
% ref point 
\addplot[only marks, mark=diamond*, mark size=2.6pt, black] coordinates {(3.300000,0)};
\addplot[black, dashed] coordinates {(3.300000,-0.06) (3.300000,0.09)};
\addplot[black, dotted] coordinates {(3.400000,-0.06) (3.400000,0.09)};
\addplot[black, densely dotted] coordinates {(2.95,0) (3.60,0)};
%%%%%%%%%%%%%%%%%%
\node[anchor=north west, font=\footnotesize] at (rel axis cs:0.02,0.98)
  {ref: $\epsilon_0=0.10$, $L_0\approx3.30$};
\node[anchor=north west, font=\footnotesize] at (rel axis cs:0.02,0.90)
  {best (full scan): $\epsilon_0\approx0.091$, $L_0\approx3.40$};

\end{axis}
\end{tikzpicture}


==> figures/tikz_export/Wide_range_Prior_sweep_BP4/fig4_adjusted.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=\columnwidth,
    height=0.63\columnwidth,
    xmode=log,
    ymode=log,
    xmin=1e-2, xmax=1e-1,
    ymin=1e-4, ymax=1,
    xlabel={\textbf{epsilon $\boldsymbol{\eps}$}},
    xlabel style={
    at={(axis description cs:0.5,0.01)},
    anchor=north
    },
    ylabel={\textbf{FER}},
    label style={font=\bfseries\small},
    tick label style={font=\tiny},
    label style={font=\scriptsize},
    grid=major,
    major grid style={gray!20},
    legend style={
        font=\scriptsize,
        at={(0.97,0.03)},
        anchor=south east,
        draw=none,
        fill=white,
        fill opacity=0.85,
        text opacity=1
    },
    legend cell align=left,
]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Worst case
\addplot[thin, red, mark=o, mark size=3pt,
         mark options={solid, fill=white},
         mark repeat=2]
    table {figures/tikz_export/fig105_curves/curve_01.dat};
\addlegendentry{$\eps_0=0.75$}
% Optimal region (main curve)
\addplot[thick, blue, mark=triangle*, mark size=3pt,
         mark repeat=2]
    table {figures/tikz_export/fig105_curves/curve_03.dat};
\addlegendentry{$\eps_0=0.091$}
%%%%%%%%%%%%%%%%%%%
\addplot[thick, green, dashed, mark=square*, mark size=1pt,
         mark repeat=2]
    table {figures/tikz_export/fig105_curves/curve_04.dat};
\addlegendentry{$\eps_0=0.10$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other mismatches 
\addplot[thick, black!60, dotted, mark=none, mark size=2pt, mark repeat=2]
    table {figures/tikz_export/fig105_curves/curve_02.dat};
\addlegendentry{$\eps_0=0.12$}

\addplot[thick, black!50, dashdotted, mark=none, mark size=2pt, mark repeat=2]
    table {figures/tikz_export/fig105_curves/curve_05.dat};
\addlegendentry{$\eps_0=0.07$}

\addplot[thick, black!90, densely dashed, mark=+, mark size=3pt, mark repeat=2]
    table {figures/tikz_export/fig105_curves/curve_06.dat};
\addlegendentry{$\eps_0=0.03$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{axis}
\end{tikzpicture}

==> figures/tikz_export/bp4_ep0_study/fig_bp4_tuneL0_a.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}

\definecolor{blueMain}{RGB}{31,119,180}
\definecolor{blueFill}{RGB}{180,200,235}
\definecolor{greenGood}{RGB}{0,150,90}
\definecolor{redBad}{RGB}{200,60,60}

\begin{axis}[
    width=0.48\textwidth,
    height=0.42\textwidth,
    grid=major,
    xlabel={$L_0$ prior strength ($\epsilon_0$ shown below)},
    ylabel={$J(L_0)=\sum_k w_k \log_{10}(\hat{p})$},
    ymin=-0.9, ymax=0,
    xmin=2, xmax=5,
    legend style={font=\footnotesize, at={(0.98,0.98)}, anchor=north east},
    title={BP4 mismatch with 95\% confidence interval},
    every axis plot/.append style={line width=0.9pt},
]

% CI band
\addplot[name path=upper, draw=none] file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_J_vs_L0_CI_high.txt};
\addplot[name path=lower, draw=none] file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_J_vs_L0_CI_low.txt};
\addplot[blueFill, fill opacity=0.35] fill between[of=upper and lower];

% Mean objective
\addplot[color=blueMain, mark=o, mark size=2.2pt]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_J_vs_L0_mean.txt};
\addlegendentry{objective mean}

% Best
\addplot[only marks, mark=square*, mark size=3.2pt]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_J_vs_L0_best.txt};
\addlegendentry{best}

% Reference ep=0.1
\addplot[only marks, mark=diamond*, mark size=3pt]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_J_vs_L0_ref.txt};
\addlegendentry{reference $\epsilon_0=0.10$}

% INSET 
\node[anchor=north east] at (rel axis cs:0.68,0.80) {
\begin{tikzpicture}
\begin{axis}[
    width=0.46\linewidth,
    height=0.38\linewidth,
    xmin=3.0, xmax=3.7,
    ymin=-0.06, ymax=0.08,
    grid=major,
    title={Zoom: $\Delta J(L_0)=J(L_0)-J(L_{0,\mathrm{ref}})$},
    xlabel={$L_0$ ($\epsilon_0$ shown below)},
    ylabel={$\Delta J(L_0)$},
    tick label style={font=\scriptsize},
    title style={font=\scriptsize},
    label style={font=\scriptsize},
]

% CI band
\addplot[name path=du, draw=none]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_dJ_vs_L0_pos.txt};
\addplot[name path=dl, draw=none]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_dJ_vs_L0_neg.txt};
\addplot[blueFill, fill opacity=0.4] fill between[of=du and dl];
% ΔJ < 0 (better)
\addplot[color=greenGood, mark=o, mark size=1.8pt]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_dJ_vs_L0_neg.txt};
% ΔJ > 0 (worse)
\addplot[color=redBad, mark=o, mark size=1.8pt]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_dJ_vs_L0_pos.txt};

\addplot[dashed] coordinates {(3.0,0) (3.7,0)};

\node[anchor=south west, font=\scriptsize] at (rel axis cs:0.02,0.02)
{$\Delta J<0$ better than ref; $\Delta J>0$ worse};
\end{axis}
\end{tikzpicture}
};
\end{axis}
\end{tikzpicture}
\caption{Prior-mismatch tuning. (a) Objective $J(L_0)$ with $95\%$ confidence interval. The optimum corresponds to a broad plateau of near-equivalent priors. Inset shows relative objective $\Delta J(L_0)$ w.r.t.\ $\epsilon_0=0.10$.}
\label{fig:bp4_tuneL0_a}
\end{figure}


==> figures/tikz_export/bp4_ep0_study/fig_bp4_tuneL0_b.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}

\definecolor{blueMain}{RGB}{31,119,180}
\definecolor{orangeMain}{RGB}{255,127,14}
\definecolor{blueFill}{RGB}{180,200,235}

\begin{axis}[
    width=0.48\textwidth,
    height=0.42\textwidth,
    grid=major,
    xlabel={$L_0$ prior strength ($\epsilon_0$ shown below)},
    ylabel={$J(L_0)$},
    xmin=2, xmax=5,
    ymin=-2, ymax=0,
    legend style={font=\footnotesize, at={(0.98,0.45)}, anchor=east},
    title={Tuning objective dominated by the low-$\epsilon$ subset},
    every axis plot/.append style={line width=0.9pt},
]

\addplot[color=blueMain, mark=o, mark size=2.2pt]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_J_vs_L0_low_eps.txt};
\addlegendentry{smaller $\epsilon$ subset ($\epsilon\le0.05$)}

\addplot[color=orangeMain, mark=square*, mark size=2pt]
    file {figures/tikz_export/bp4_ep0_study/data_txt/BP4_J_vs_L0_high_eps.txt};
\addlegendentry{larger $\epsilon$ subset ($\epsilon>0.05$)}

\end{axis}
\end{tikzpicture}
\caption{Split objective. Sensitivity to the assumed prior is dominated by the low-noise ($\epsilon$) regime, while the high-$\epsilon$ subset remains comparatively flat.}
\label{fig:bp4_tuneL0_b}
\end{figure}

